Transfer Function Models for Cylindrical MC Channels with Diffusion and Laminar Flow

The analysis and design of advection-diffusion based molecular communication (MC) systems in cylindrical environments is of particular interest for applications such as micro-fluidics and targeted drug delivery in blood vessels. Therefore, the accurate modeling of the corresponding MC channel is of high importance. The propagation of particles in these systems is caused by a combination of diffusion and flow with a parabolic velocity profile, i.e., laminar flow. The propagation characteristics of the particles can be categorized into three different regimes: The flow dominant regime where the influence of diffusion on the particle transport is negligible, the dispersive regime where diffusion has a much stronger impact than flow, and the mixed regime where both effects are important. For the limiting regimes, i.e., the flow dominant and dispersive regimes, there are well-known solutions and approximations for particle transport. In contrast, there is no general analytical solution for the mixed regime, and instead, approximations, numerical techniques, and particle based simulations have been employed. In this paper, we develop a general model for the advection-diffusion problem in cylindrical environments which provides an analytical solution applicable in all regimes. The modeling procedure is based on a transfer function approach and the main focus lies on the incorporation of laminar flow into the analytical model. The properties of the proposed model are analyzed by numerical evaluation for different scenarios including the uniform and point release of particles. We provide a comparison with particle based simulations and the well-known solutions for the limiting regimes to demonstrate the validity of the proposed analytical model.

==> inputs.tex <==
\subsection{Initial Conditions}

\subsection{External Sources}

\subsubsection{Temporal Pulses}

\subsubsection{Spatial Shapes}

==> misc.tex <==
\subsubsection{Temporal shaping} Three different temporal pulses are considered for the temporal shape $f_\mathrm{temp}(t)$ of $f_\mathrm{s}$ in \eqref{eq:60}, that are defined by their temporal center position $t_\mathrm{e}$ and their width $t_0$ and an overview is given in Figure~\ref{fig:5}. The most common temporal pulse shape is an individual impulse at a certain time $t_\mathrm{e}$, i.e., 
\begin{align}
	&f_\mathrm{temp}(t) = f_1(t) = \delta(t - t_\mathrm{e}), &t_\mathrm{e} > 0. \label{eq:73}
\end{align}
	The second considered temporal shape is an rectangular shape of width $t_0$ and centered at $t_\mathrm{e}$
\begin{align}
	&f_\mathrm{temp}(t) =f_2(t) = \mathrm{rect}\left(\frac{t - t_\mathrm{e}}{t_0}\right), &t_\mathrm{e} > \frac{t_0}{2}. \label{eq:74}
\end{align}
The temporal shapes \eqref{eq:73}, \eqref{eq:74} are very common, but both rely on the unrealistic assumption of instantaneous particle release (slopes of the rectangular function). Therefore, a third temporal shape is assumed to model a more realistic release of particles. As shown in Figure~\ref{fig5:fig3} a raised cosine function is considered
\begin{align}
	&f_\mathrm{temp}(t) = f_3(t) = 
	\begin{cases}
		\frac{1}{2}\left(1 +\cos(\omega_0(t - t_\mathrm{e})) \right) & t_\mathrm{e}-\frac{t_0}{2} \le t \le t_\mathrm{e}+\frac{t_0}{2}\\
		0 & \mathrm{else}
	\end{cases},\label{eq:75}
\end{align}
with $\omega_0 = \frac{2\pi}{t_0}$.

\subsubsection{Spatial shaping} Two different spatial distributions are considered for the spatial shape of initial conditions $p_\mathrm{i}$ in \eqref{eq:59} and for the spatial shaping $f_\mathrm{spat}(\bm{x})$ of $f_\mathrm{s}$ in \eqref{eq:60}. The first considered shape is a spatial impulse, defined in terms of a 3D delta impulse at $\bm{x}_\mathrm{e} = \left[r_\mathrm{e}, \varphi_\mathrm{e}, z_\mathrm{e}\right]\tran$
\begin{align}
	f_\mathrm{spat}(\bm{x}) = f_1(\bm{x}) = \delta(r - r_\mathrm{e})\delta(\varphi - \varphi_\mathrm{e})\delta(z - z_\mathrm{e}). \label{eq:76}
\end{align}
An impulse release of particles as in \eqref{eq:76} is not very practical, therefore a spatial distribution with a non-zero volume is defined in terms of a function $f_r$ in radial direction and a function $f_z$ in $z$-direction, respectively, while the delta impulse in angular direction persists
\begin{align}
	f_\mathrm{spat}(\bm{x}) = f_2(\bm{x}) = f_r(r)f_\varphi(\varphi)f_z(z). \label{eq:77}
\end{align}
The functions $f_r$, $f_\varphi$, $f_z$ can be defined arbitrarily to realize a specific spatial distribution of particles. The function $f_r$ and $f_\varphi$ are varied, but the function $f_z$ is defined in terms of a raised cosine function centered at $z_\mathrm{e}$ and a width of $z_0$
\begin{align}
	f_z(z) &= \begin{cases}
		\frac{1}{2}( 1 + \cos(k_z(z - z_\mathrm{e}))) & 
		z_\mathrm{e} - \frac{z_0}{2} \le z \le z_\mathrm{e} + \frac{z_0}{2}
		\\0 & \mathrm{else}
	\end{cases},\label{eq:78}
\end{align}
with $k_z = \frac{2\pi}{z_0}$. This function is chosen to obtain a smooth distribution of particles in $z$-direction to avoid the presence of Gibb's phenomenon as discussed in Section~\ref{}.

The functions $f_r$ and $f_\varphi$ are given for two different forms of particle distribution. A common example is a distribution of particles in a circular disk with radius $r_0$ (see e.g.~\cite{jamali:ieee:2019, wicke:globecom:2018}), i.e.,  
\begin{align}
	&f_r(r) = \mathrm{rect}\left(\frac{r}{r_0}\right), & f_\varphi(\varphi) = 1.
	\label{eq:79}
\end{align}
	Furthermore, we assume a point release of particles with a spreading in radial direction, i.e., 
\begin{align}
	&f_r(r) = \begin{cases}
		\frac{1}{2}( 1 + \cos(k_r(r - r_\mathrm{e}))) & 
		r_\mathrm{e} - \frac{r_0}{2} \le r \le r_\mathrm{e} + \frac{r_0}{2}\\
		0 & \mathrm{else}
	\end{cases}, 
	&f_\varphi(\varphi) = \delta(\varphi -\varphi_\mathrm{e}), \label{eq:80}
\end{align}
with $k_r = \frac{2\pi}{r_0}$.

==> modeling_procedure.tex <==
Before the modeling of the considered system in Figure~\ref{fig:1} is presented in Sections~\ref{sec:tfm1} and \ref{sec:tfm2}, this section introduces the overall modeling procedure as shown in Figure~\ref{fig:2}.
%
As mentioned in the Introduction, there are no comprehensive models for the transport of particles by diffusion and laminar flow in a cylindrical environment. Despite the simplification of the initial transport equation \eqref{eq:4} direct solutions for the system in \eqref{eq:7}, \eqref{eq:8} have so far not been found to the best knowledge of the authors. 
%


%
Instead of the direct solution of \eqref{eq:7}, \eqref{eq:8} we propose a modeling procedure as shown in Figure~\ref{fig:2}. 
%
Starting point for the modeling procedure is the vector-valued IBVP of the considered problem in the $s$-domain \eqref{eq:22}--\eqref{eq:24}, where the term responsible for the laminar flow $\bm{v}_\mathrm{flow}$ is arranged as an external source in the vector $\bm{F}_\mathrm{e}$. This vector can be decomposed into 
\begin{align}
\bm{F}_\mathrm{e}(\bm{x},s) = \bm{F}_\mathrm{q}(\bm{x},s) + \bm{F}_\mathrm{flow}(\bm{x},s) = 
\begin{bmatrix}
\bm{0}\\
F_\mathrm{s}(\bm{x},s)
\end{bmatrix} + 
\begin{bmatrix}
\bm{V}_\mathrm{flow}(\bm{x},s)\\
0
\end{bmatrix} \label{eq:25a}, 
\end{align}
where $\bm{F}_\mathrm{q}$ contains the external source function $F_\mathrm{s}(\bm{x},s)$ in the $s$-domain and $\bm{F}_\mathrm{flow}$ contains the term $\bm{V}_\mathrm{flow}(\bm{x},s)$ that is responsible for the attraction of particles by laminar flow. 

As a first step, the influence of the term $\bm{F}_\mathrm{flow}$ is omitted yielding a simplification of the scenario to a 3D diffusion problem in the cylinder of volume $V$. 
%
In Section~\ref{sec:tfm1} the simplified 3D diffusion system is modeled by a transfer function approach and finally formulated in terms of a SSD, i.e., the open loop SSD. 
%
By techniques related to control theory (see \cite{Deutscher:book:2012}) and the incorporation of complex boundary conditions (see \cite{schaefer:icc:2019, rabenstein:ijc:2017}), the influence of the excluded flow term $\bm{v}_\mathrm{flow}$ on the system is reduced to an influence on the eigenvalues of the system. 
%
Finally, in Section~\ref{sec:tfm2} the excluded and reformulated flow terms are reincorporated into the open loop SSD model of the 3D diffusion process yielding the closed loop SSD model of the considered 3D advection-diffusion process with laminar flow profile. 
% 
%The terms \textit{open loop} and \textit{closed loop} are chosen in correspondence to control theory. This is because the reincorporation of $\bm{v}_\mathrm{flow}$ establishes a feedback loop that is attached to the open loop model of the diffusion process (see Figure~\ref{???} in Section~\ref{sec:tfm2})

\begin{figure}[t]
	\centering
	\scalebox{0.9}{
	\begin{tikzpicture}[
	box/.style={rectangle,draw,thick,rounded corners, text width=2cm,minimum height=10mm, node distance=1mm, align=center},
	arrow/.style={-latex,thick,draw,rounded corners}
	]
	%				\draw[help lines] (-7,0) grid (7,-18);
	%	\node[box, text width=5cm,fill=blue!10] (3d) 	at (0,0) {\small $3$D Cylinder: \\diffusion, flow, mag. force};
	%	\node[box] (2d) [below = 15mm of 3d, text width=5cm,fill=blue!10]{\small $2$D Circular Disk:\\ diffusion, mag. force};	
	\node[box] (3d) [text width=8cm]  at (0,0) {3D Cylinder \\Diffusion + Laminar Flow\\ $\left[s\bm{C} - \Lp\right]\bm{Y}(\bm{x},s) = \bm{F}_\mathrm{q}(\bm{x},s) + \bm{F}_\mathrm{flow}(\bm{x},s)$};
	\node[box] (3d2) [below= 30mm of 3d, text width=5cm]  at (0,0) {3D Cylinder \\Diffusion + \textbf{no} Flow\\ $\left[s\bm{C} - \Lp\right]\bm{Y}(\bm{x},s) = \bm{F}_\mathrm{q}(\bm{x},s)$};
	\node[box] (modelSBC) [below= 20mm of 3d2, text width=5cm] {Open loop TFM: \\ Cylinder with Diffusion};
	\node[box] (modelCBC)  [below = 20mm of modelSBC, text width=5cm] {Closed Loop TFM:\\ Cylinder with Diffusion + Laminar flow};
	%	\node[box] (modelSim)  [below = 15mm of modelCBC, text width=5cm,fill=red!20] {Simulation model SSD\\ string with complex BCs};
	
	\node[box] (fb)  [below right= 2mm and 20mm of 3d, text width=4cm] {Laminar flow\\
		$v(r) = 2v_\mathrm{eff}\left(1 - \frac{r^2}{R_0^2}\right)$};
	
	\node[box] (fb1)  [below left= 15mm and -10mm of fb, text width=3cm] {Uniform flow\\
		$v_\mathrm{uni} = 2v_\mathrm{eff}$};
	\node[box] (fb2)  [below right= 15mm and -10mm of fb, text width=3cm] {Laminar profile\\
		$v_\mathrm{lam} = -2v_\mathrm{eff}\frac{r^2}{R_0^2}$};
	\node[coordinate] (a) [below = 12mm of fb]{};	
	\node[coordinate] (b) [below = 10mm of modelSBC]{};
	\draw[arrow] (3d)   -- node[left]{\small $\bm{F}_\mathrm{flow}(\bm{x},s) = \bm{0}$} (3d2);
	\draw[arrow] (3d)   |- (fb);
	
	\draw[arrow] (modelSBC)   -- node[left]{\small Modeling (Section~\ref{sec:tfm2})} (modelCBC);
	\draw[] (fb) --node[left]{\small Decompose} (a);
	\draw[arrow] (3d2) -- node[left]{\small Modeling (Section~\ref{sec:tfm1})} (modelSBC);
	\draw[arrow] (fb)   |-  (fb1);
	\draw[arrow] (fb)   |- (fb2);
	\draw[thick] (fb1)  |- (b);	
	\draw[thick] (fb2)   |- (b);
	\end{tikzpicture}
	}
	\caption{Modeling procedure for the system shown in Fig.~\ref{fig:1} including diffusion and flow in a cylindrical environment.}
	\label{fig:2}
\end{figure}

==> tikzlibrarydsp.code.tex <==
% -------------------------------------------------------------------------
% This library for block diagrams and signal flow graphs was inspired by
% the library "signalflow" of Dr. Karlheinz Ochs, Ruhr-University of Bochum,
% Germany. Furthermore, some ideas were taken from the library "circuitikz"
% of Massimo A. Redaelli and from the PGF library itself.
%
% Copyright 2012 by Matthias Hotz
%
% This work is licensed under the Creative Commons Attribution 2.5 Generic
% License. To view a copy of this license, visit
%          http://creativecommons.org/licenses/by/2.5/
% or send a letter to Creative Commons, 444 Castro Street, Suite 900,
% Mountain View, California, 94041, USA.
% -------------------------------------------------------------------------

\usetikzlibrary{arrows, calc, positioning, decorations.markings}

% -------------------------------------------------------------------------
% Parameters for the library

\newcommand{\dsplinewidth}{0.25mm}           % Line width for connections
\newcommand{\dspblocklinewidth}{0.3mm}       % Line width for blocks
\newcommand{\dspoperatordiameter}{4mm}       % Diameter for adder, multiplier, mixer
\newcommand{\dspoperatorlabelspacing}{2mm}   % Distance from symbol to label for adder, multiplier, mixer
\newcommand{\dspnoderadius}{1mm}             % Filled and empty node
\newcommand{\dspsquareblocksize}{8mm}        % Size for square blocks, e.g. for delay elements, decimator, expander
\newcommand{\dspfilterwidth}{14mm}           % Width of a filter block

% -------------------------------------------------------------------------
% Define new arrow heads

\pgfarrowsdeclare{dsparrow}{dsparrow}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt} % Solid line (do not dash)
	\pgfsetmiterjoin	 % Fixed miter join of line
	\pgfsetbuttcap		 % Fixed butt cap of line
	\pgfpathmoveto{\pgfpoint{-4\arrowsize}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{4\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{-4\arrowsize}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

\pgfarrowsdeclare{dsparrowmid}{dsparrowmid}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt}
	\pgfsetmiterjoin
	\pgfsetbuttcap
	\pgfpathmoveto{\pgfpoint{0}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{8\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{0}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

% -------------------------------------------------------------------------
% Define new node shapes

\makeatletter

\pgfkeys{/tikz/dsp/label/.initial=above}

% Generic shape generator for operators, i.e. nodes with a circular
% shape with an additional customizable drawing and a text label
\long\def\dspdeclareoperator#1#2{
	\pgfdeclareshape{#1}
	{
		% Saved anchors, macros and dimensions
		\savedanchor\centerpoint{\pgfpointorigin}
		\savedmacro\label{\def\label{\pgfkeysvalueof{/tikz/dsp/label}}}
	  \saveddimen\radius
	  {
		  \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
		  \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
	    \ifdim\pgf@xa>\pgf@ya
	      \pgf@x=.5\pgf@xa
	    \else
	      \pgf@x=.5\pgf@ya
	    \fi
	  }
	  
	  % Inherit all anchors from the 'circle'-shape:
	  \inheritanchor[from={circle}]{center}
	  \inheritanchor[from={circle}]{mid}
	  \inheritanchor[from={circle}]{base}
	  \inheritanchor[from={circle}]{north}
	  \inheritanchor[from={circle}]{south}
	  \inheritanchor[from={circle}]{west}
	  \inheritanchor[from={circle}]{east}
	  \inheritanchor[from={circle}]{mid west}
	  \inheritanchor[from={circle}]{mid east}
	  \inheritanchor[from={circle}]{base west}
	  \inheritanchor[from={circle}]{base east}
	  \inheritanchor[from={circle}]{north west}
	  \inheritanchor[from={circle}]{south west}
	  \inheritanchor[from={circle}]{north east}
	  \inheritanchor[from={circle}]{south east}
	  \inheritanchorborder[from={circle}]
	  
	  % Draw circle and embed additional code
	  \backgroundpath
	  {
	    % Draw circle
	    \pgfpathcircle{\centerpoint}{\radius}
	    
	    % Embed additional code
	    % (Note that this code must call e.g. \pgfusepathqstroke
	    #2
	  }
	
		% Define anchor parametrized by the PGF key /tikz/dsp/label
	  \anchor{text}
	  {
			\centerpoint
			%
	    \def\templabelabove{above}
	    \def\templabelbelow{below}
	    \def\templabelleft{left}
	    \def\templabelright{right}
	    \pgfutil@tempdima=\dspoperatorlabelspacing
	    %
	    \ifx\label\templabelabove
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by \radius
				\advance\pgf@y by \pgfutil@tempdima
	    \fi
	    %
	    \ifx\label\templabelbelow
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by -\radius
				\advance\pgf@y by -\pgfutil@tempdima
				\advance\pgf@y by -\ht\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelleft
				\advance\pgf@x by -\radius
				\advance\pgf@x by -\pgfutil@tempdima
				\advance\pgf@x by -\wd\pgfnodeparttextbox
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelright
				\advance\pgf@x by \radius
				\advance\pgf@x by \pgfutil@tempdima
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	  }
	}
}

\dspdeclareoperator{dspshapecircle}{\pgfusepathqstroke}

\dspdeclareoperator{dspshapecirclefull}{\pgfusepathqfillstroke}

\dspdeclareoperator{dspshapeadder}{
	% Coordinate offset for the plus
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.55\pgfutil@tempdima
	
	% Draw plus
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{0pt}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{0pt}}}
	
	\pgfusepathqstroke
}

\dspdeclareoperator{dspshapemixer}{
	% Coordinate offset for the cross
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.707106781\pgfutil@tempdima
	
	% Draw cross
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{ \pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{-\pgfutil@tempdima}}}
	
	\pgfusepathqstroke
}

\makeatother

% -------------------------------------------------------------------------
% Define node styles

\tikzset{dspadder/.style={shape=dspshapeadder,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmultiplier/.style={shape=dspshapecircle,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmixer/.style={shape=dspshapemixer,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}

\tikzset{dspnodeopen/.style={shape=dspshapecircle,line width=\dsplinewidth,minimum size=\dspnoderadius}}
\tikzset{dspnodefull/.style={shape=dspshapecirclefull,line width=\dsplinewidth,fill,minimum size=\dspnoderadius}}

% The fixed specification of text height and text depth is the somewhat
% unaesthetic workaround to align the text in different node at the same
% baseline. See the PGF/TikZ manual, ch. 5.1.
\tikzset{dspsquare/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum size=\dspsquareblocksize}}
\tikzset{dspfilter/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum height=\dspsquareblocksize,minimum width=\dspfilterwidth}}

% -------------------------------------------------------------------------
% Define "signal flow" lines

\tikzset{dspline/.style={line width=\dsplinewidth},line cap=round,line join=round}
\tikzset{dspconn/.style={->,>=dsparrow,line width=\dsplinewidth},line cap=round,line join=round}%line cap=rect,line join=miter}
\tikzset{dspflow/.style={line width=\dsplinewidth,line cap=round,line join=round,
  decoration={markings,mark=at position 0.5 with {\arrow{dsparrowmid}}},postaction={decorate}}}

% -------------------------------------------------------------------------
% Define various utility macros

\newcommand{\downsamplertext}[1]{\raisebox{0.1em}{$\big\downarrow$}#1}
\newcommand{\upsamplertext}[1]{\raisebox{0.1em}{$\big\uparrow$}#1}

